Shapely monads and analytic functors

In this paper, we give precise mathematical form to the idea of a structure whose data and axioms are faithfully represented by a graphical calculus; some prominent examples are operads, polycategories, properads, and PROPs. Building on the established presentation of such structures as algebras for monads on presheaf categories, we describe a characteristic property of the associated monads---the shapeliness of the title---which says that "any two operations of the same shape agree". An important part of this work is the study of analytic functors between presheaf categories, which are a common generalisation of Joyal's analytic endofunctors on sets and of the parametric right adjoint functors on presheaf categories introduced by Diers and studied by Carboni--Johnstone, Leinster and Weber. Our shapely monads will be found among the analytic endofunctors, and may be characterised as the submonads of a universal analytic monad with "exactly one operation of each shape". In fact, shapeliness also gives a way to define the data and axioms of a structure directly from its graphical calculus, by generating a free shapely monad on the basic operations of the calculus. In this paper we do this for some of the examples listed above; in future work, we intend to do so for graphical calculi such as Milner's bigraphs, Lafont's interaction nets, or Girard's multiplicative proof nets, thereby obtaining canonical notions of denotational model.

==> stacey.tex <==


\makeatletter
\pgfkeys{
  /pgf/scalable arrows/.code={
    \let\pgf@add@arrows@as@needed=\pgf@add@scalable@arrows@as@needed
    \let\pgf@shorten@path@as@needed=\pgf@shorten@path@as@needed@for@scalable
  },
  /pgf/arrow scale factor/.initial=1,
}

\def\pgf@add@scalable@arrows@as@needed{%
  \pgfkeysgetvalue{/pgf/arrow scale factor}{\pgf@temp}%
  \let\pgf@restorelw=\pgfutil@empty
  \ifx\pgf@temp\pgfutil@empty
  \else
  \edef\pgf@restorelw{\noexpand\pgfsetlinewidth{\the\pgflinewidth}}%
  \pgfsetlinewidth{\pgf@temp\pgflinewidth}%
  \fi
  \ifx\pgf@startarrow\pgfutil@empty%
  \else%
    \pgflowlevelobj%
      {\pgftransformarrow{\pgfpointsecondonpath}{\pgfpointfirstonpath}}
      {\pgf@startarrow}%
  \fi%
  \ifx\pgf@endarrow\pgfutil@empty%
  \else%
    \pgflowlevelobj%
      {\pgftransformarrow{\pgfpointsecondlastonpath}{\pgfpointlastonpath}}
      {\pgf@endarrow}%
  \fi%
      \pgf@restorelw%
}

\def\pgf@shorten@path@as@needed@for@scalable{%
  \pgfkeysgetvalue{/pgf/arrow scale factor}{\pgf@temp}%
  \let\pgf@restorelw=\pgfutil@empty
  \ifx\pgf@temp\pgfutil@empty
  \else
  \edef\pgf@restorelw{\noexpand\pgfsetlinewidth{\the\pgflinewidth}}%
  \pgfsetlinewidth{\pgf@temp\pgflinewidth}%
  \fi
  \pgfprocesspathextractpoints{\pgf@arrowpath}%
  \let\pgf@arrow@next=\pgf@shorten@now%
  \ifx\pgf@shorten@start\pgfutil@empty%
    \ifx\pgf@shorten@end\pgfutil@empty%
      \ifdim\pgf@shorten@end@additional=0pt\relax%
        \ifdim\pgf@shorten@start@additional=0pt\relax%
          \let\pgf@arrow@next=\relax%
        \fi%
      \fi%
    \fi%
  \fi%
  \pgf@arrow@next%
  \pgf@restorelw%
}

\makeatother
